"A Good Bot Always Knows Its Limitations": Assessing Autonomous System Decision-making Competencies through Factorized Machine Self-confidence

How can intelligent machines assess their competency to complete a task? This question has come into focus for autonomous systems that algorithmically make decisions under uncertainty. We argue that machine self-confidence -- a form of meta-reasoning based on self-assessments of system knowledge about the state of the world, itself, and ability to reason about and execute tasks -- leads to many computable and useful competency indicators for such agents. This paper presents our body of work, so far, on this concept in the form of the Factorized Machine Self-confidence (FaMSeC) framework, which holistically considers several major factors driving competency in algorithmic decision-making: outcome assessment, solver quality, model quality, alignment quality, and past experience. In FaMSeC, self-confidence indicators are derived via 'problem-solving statistics' embedded in Markov decision process solvers and related approaches. These statistics come from evaluating probabilistic exceedance margins in relation to certain outcomes and associated competency standards specified by an evaluator. Once designed, and evaluated, the statistics can be easily incorporated into autonomous agents and serve as indicators of competency. We include detailed descriptions and examples for Markov decision process agents, and show how outcome assessment and solver quality factors can be found for a range of tasking contexts through novel use of meta-utility functions, behavior simulations, and surrogate prediction models. Numerical evaluations are performed to demonstrate that FaMSeC indicators perform as desired (references to human subject studies beyond the scope of this paper are provided).

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

==> competency_formalization.tex <==
\subsection{Formalization}\label{sec:formalization}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\columnwidth]{figs/competency_fig.png}
\caption{\nra{...to write caption later}}
%\caption{Factors and relationships in computational competency evaluation: a competency indicator function $f_i$ compares a competency standard $\Sigma_i$ (determined by the Evaluator) against outcomes, states, and signals ($O, S, \Gamma_a, \Delta_a$) that describe the Agent's capabilities, conditioned on evaluation context variables ($C,A,E,\Theta, \Lambda_a$) which the Agent cannot affect. \nra{include `consequence' arrows for comp eval? similar to Brett's thesis: what gets done with comp eval?}\bi{how important do we think this symbolic notation is going to be in the future. If we think it's going to be important and re-used we may want to iterate a couple of times to carefully choose symbols and superscripts/subscripts. On the other hand if we don't think we'll re-use it (or that others will) often then perhaps it doesn't matter as much. One example is superscripts $i$ and $f$ for 'initial' and 'final'. We might also consider $0$ and $N$ or something else\ldots also, I tend to think of dashed lines as more mutable (dynamic) than solid ones, but I'll defer to you if you're following a standard/preference I'm not aware of}}
\label{fig:CompAssessGenBlockDiag}
\end{figure}

Figure \ref{fig:CompAssessGenBlockDiag} illustrates the relationships that generally exist between the \emph{Agent}, \emph{Environment}, \emph{Task Context}, \emph{Signals of interest}, and \emph{Outcomes of interest} which inform the computation of a single \emph{Competency Indicator Function} $f_i$ with respect to competence standard $\Sigma_i$. The dashed arrows in this figure denote pre-determined or static relationships that involve information not expected to evolve as a result of $A$'s operation \nra{should change aua to be possibly dynamic or mixed? dynamic user interaction...}, whereas the solid arrows denote changeable/dynamic relations involving information that can vary over the course of $A$'s operation. %%a0 should stay fixed even for meta-reasoning agent: still have ability to watch/change s_a via a_aa, so a0 just means the parameters needed to realize an instantiation of a specific meta-reasoning agent...
The italicized terms above are now defined:

\begin{description}
\item[Agent ($A$):] consists of the computational elements which allow a delegated machine entity to decide and act under its own auspices to perform a task - that is, to achieve a desired $O$, in a given $E$ while operating under $C$. In this sense, $A$ corresponds to the combined set of internal models, signals, algorithms, and associated assumptions and approximations used for machine reasoning, knowledge representation, planning, learning, perception, motion/execution, and communication in a decision making problem. This excludes the physical machine manifestation (i.e. software and hardware implementations), but accounts for sources of dynamic computational behavior, which can be described by states $\vec{s}_a$. 

\item[Environment ($E$):] the domain of variables which completely describes the task evolution and in which outcomes of interest $O$ are produced as a result of decisions made by $A$, subject to $C$. Here $E$ embodies the real world setting in which the task takes place, and describes all variables and associated dynamics which are external to $A$ (and its specification) yet relevant to determining $O$ while being subject to $C$. Let $\vec{s}_e$ be the dynamic state of these variables. Although realistically $\vec{s}_e$ is at best only partly known to $A$ and the Evaluator (i.e. `unknown unknowns' often exist from the perspective of either), it is assumed here -- for the sake of building a simple but rigorous computational competency evaluation framework-- that $\vec{s}_e$ describes all relevant factors and is available to the Evaluator. The set $\theta_{cf}$ represents function mappings from $\vec{s}_e$ to $O$. The impact of `unknown unknowns' will be considered later.  %As will be shown later in the running application examples, the extent to which $A$ can access $\vec{s}_e$ depends on $A$'s design. \nra{interesting implications for self-assessment, since it raises the possibility that $A$/Evaluator may not be competent enough at competency assessment -- worth commenting on later...this also is why we look at it from the external eval point of view...}
%%Importantly, $C$ includes variations and changing dynamics that influence the ability of an agent to act.

\item[Task Context ($C$):] contains all information needed to completely specify %(i.e. contextualize) 
a single decision making problem instance, in which $A$ attempts to achieve a desirable $O$ in $E$. This includes: the configuration of $E$; constraints governing $E$'s evolution (denoted by the set $\theta_{ce}$) and definition/constraints of $O$ as it pertains to the task (denoted by the set $\theta_{cf}$); initial conditions for states describing temporal dynamics of $E$ and $A$ (denoted $\vec{s}^i_e$ and $\vec{s}^i_a$); and $A$'s overall physical manifestation (software/hardware substrates). Excluded are parameters, data, and other signals $\alpha_{0a}$ selected for/sent to $A$ at run time, such as training data or free algorithm parameters (e.g. tuning knobs like convergence tolerances, hyper-parameters, etc.), as well as inputs $\alpha_{ua}$ supplied by external users, operators, or evaluators (e.g. commands, requests, responses to machine queries, etc.). %%alpha0a can induce minor changes in which `version' of same $A$ attempts the task given same $C$ and $E$... 

\item[Outcomes of interest ($O$):] set of variables that describe desired results of task completion as a function of $\vec{s}_e$ and $C$, where the set $\theta_{ef}$ denotes mappings from $\vec{s}_e$ to $O$. Related to (but distinct from) these are desired final configurations of $E$ and $A$, respectively denoted $\vec{s}^f_e$ and $\vec{s}^f_a$. The problem of assessing the extent to which instances of $O$, $\vec{s}^f_e$, and $\vec{s}^f_a$ can be achieved/changed via $A$'s actions lies at the heart of computational competency evaluation.  Here, the term ``of interest'' highlights the fact that there is not necessarily a single outcome on which competency evaluation is based. Outcomes of interest are likely slightly less numerous than the total number of unique tasks to be performed by $A$. Some examples of typical outcomes are: training/test errors, response time, steady-state error, cumulative expected reward, objective function value, number of objects of interest retrieved, number of operator interventions, and classification accuracy. \nra{could cite SUCCESS MURI paper for other `Level 1' examples?} 
In situations where $A$ explicitly reasons over some/all elements of $O$ and $\vec{s}^f_e$, $A$ generally must acquire and process information from $E$ to do so. %%, though these elements may be more directly accessible in some cases.

\item[Signals of interest ($S,\Gamma_a,\Delta_a$)]: dynamic variables that describe the behaviors of $A$ and $E$ subject to $C$, where: $S=\left\{ \vec{s}_e,\vec{s}_a \right\}$ denotes the combined set of $E$ and $A$ states; $\Gamma_a = \left\{\gamma_{ae}, \gamma_{au} \right\}$ denotes the set of actions produced by $A$  to conduct the task; and $\Delta_a = \left\{\alpha_{ca}, \alpha_{aa}, \alpha_{ea} \right\}$ denotes the set of information $A$ gathers/produces for itself to conduct the task. 
Here, $\gamma_{ae}$ is the set of signals transmitted from $A$ to $E$ as a result of $A$'s decisions (i.e. action variables describing $A$'s effects on $E$), and $\gamma_{ua}$ is the set of signals transmitted from $A$ to a user/Evaluator (e.g. explanations of actions, warnings, prompts for input, etc.). The sets $\alpha_{aa}$ and $\alpha_{ea}$ define `closed-loop' feedback signals that allow $A$ to monitor itself (adjust $\vec{s}_a$) and $E$ (influence $\vec{s}_e$) during a task, whereas $\alpha_{ca}$ corresponds to the set of all initial `open-loop' information $A$ ingests and interprets for itself at the start of a task. Whereas the signals ($S,\Gamma_a,\Delta_a$) all originate from either $A$ or $E$, the signals in set $\Lambda_a = \left\{\alpha_{0a}, \alpha_{ua} \right\}$ come from either the user or designer. The set $\Theta = \left\{\theta_{ce}, \theta_{ef}, \theta_{cf} \right\}$ collects contextual constraints and functions as opposed to variable signals. 

\item[Competency indicator function ($f_i$)]: a mapping generally from the combined space of elements of the sets $\Sigma_i,O,S,\Gamma_a,\Delta_a$ to a space ${\mathbb S}_i$ which describes the range of possible competency statements for criterion $i=1,...,M$. 
${\mathbb S}_i$ may for instance correspond to a discrete label or a continuous competency scale. It is possible for only certain parts of $O,S,\Gamma_a,\Delta_a$ to matter for comparison against $\Sigma_i$ in evaluation, so the signature and ${\mathbb S}_i$ for $f_i$ can vary across different criteria $i$. Each $f_i$ also has a dependency on evaluation context variables, represented  in Fig. \ref{fig:CompAssessGenBlockDiag} by the vertical bar $|C, A, E, \Theta, \Lambda_a$ (read as `given $C, A, E, \Theta, \Lambda_a$'). Note that $\Sigma_i$ relates to some subset of all variables except $C, A, E, \Theta, \Lambda_a$, since these are beyond $A$'s influence. \nra{a priori, in situ, post hoc w.r.t. task performance ...}
\end{description}

These definitions and Fig. \ref{fig:CompAssessGenBlockDiag} allow us to more formally revisit the points raised in in Sec. \ref{sec:synthesis}. Firstly, it can be seen that evaluation of expected capabilities explicitly occurs in the comparison of $\Sigma_i$ to $(O,S,\Gamma_a,\Delta_a)$ via $f_i$, given an assumed setting that is captured by the dependency on $(C, A, E, \Theta, \Lambda_a)$.  
%
%\nra{to polish: insights and takeaways to expand on:} (1) separating asymmetric layers of competency/effectiveness: need to discern `intrinsic' capability [largely determined by `settings'-whether or not something is fundamentally possible and doable] from `expected capability' [determined by `effects'/degree of agency within a given setting - whether or not agent can behave as designed/intended - potential vs realized capabilities, esp for info gathering/adaptive agents that must act under uncertainty] ---  control theoretic and formal methods ideas of reachable/unreachable [observable/unobservable] tend to play more to certain notions of intrinsic capability (i.e. what's mathematically feasible and possible, even if not completely practical or realistic), but also provide insight on expected capability up to a certain point (in what way and why only up to a point?) \nra{or maybe control/formal methods are more about expected capabilities? tend to be very instance and problem specific...} 
Secondly, diving deeper into assessment of expected capabilities and recalling Daw, et al. [\nra{cite}] on the need for meta-reasoning: it is easy to see that $(O,S)$ provides `1st order' information for assessing effects of $A$'s behavior (i.e. task results - what/where are agent's effects?), while $(\Gamma_a,\Delta_a)$ provides `2nd order' information for assessing causes of $A$'s behavior (i.e. resulting behaviors -- how/why are agent's effects produced?). 
Since $\Sigma_i$ informs expected capabilities by specifying demanded task results and behaviors, 
this can be explicitly represented as $\Sigma_i = (O^*_i,S^*_i, \Gamma^*_{a,i},\Delta^*_{a,i})$, and so $f_i$ can be generically written as
\begin{align}
f_i(\Sigma_i,O,S,\Gamma_a,\Delta_a|C,A,E,\Theta,\Lambda_a) =   (O,S, \Gamma_{a},\Delta_{a}) \ominus (O^*_i,S^*_i, \Gamma^*_{a,i},\Delta^*_{a,i}),
\end{align}
where $\ominus$ denotes a comparison operation that maps to $\mathbb{S}_i$. The exact specification of $(O,S,\Gamma_a,\Delta_a)$, $\ominus$, and $\mathbb{S}_i$ depends on the competency criterion $i$. However, note that $f_i$ can also be readily defined to assess different aspects of task results and resulting behaviors separately, e.g. 
\begin{align}
    f_{1}(O^*,O|C,A,E,\Theta,\Lambda_a) &= O^* \ominus O \mapsto \mathbb{S}_1, \\
    f_{2}(S^*,S|C,A,E,\Theta,\Lambda_a) &= S^* \ominus S \mapsto \mathbb{S}_2, \\
    f_{3}(\Gamma_a^*,\Gamma_a|C,A,E,\Theta,\Lambda_a) &= \Gamma_a^* \ominus \Gamma_a \mapsto \mathbb{S}_3, \\
    f_{4}(\Delta_a^*,\Delta_a|C,A,E,\Theta,\Lambda_a) &= \Delta_a^* \ominus \Delta_a \mapsto \mathbb{S}_4,
\end{align}
which in turn could be combined into other composite competency indicators. Moreover, different subsets of $O,S,\Gamma_a,$ and $\Delta_a$ can be separately interrogated via corresponding $f_i$, $\mathbb{S}_i$ and of $\Sigma_i$. 

Thirdly, observe that a choice of ordinal spaces $\mathbb{S}_i$ permits generation of graduated competency statements, and thus assignment of \emph{ordered degrees of competency} to $A$ relative to $\Sigma_i$. 
While often desirable, this is not strictly necessary, as assessments can be made in relation to sets of categorical alternatives with partial/no ordering (e.g. `handles like a sports car' vs. `handles like a truck', etc.). Where totally ordered degrees of competency do exist, it may be convenient for $\mathbb{S}_i$ to be a finite scale with an upper/lower bound to denote maximum exceedance/deceedance of demanded capabilities, i.e. maximum/minimum achievable grades. 
In other cases, unbounded degrees of competency can be more informative, e.g. arbitrarily positive/negative stability margins for feedback control systems [\nra{cite}]. 
In any case, one may see useful analogy between competency assessment and generation of a `report card' for $A$ with respect to different `subjects' $i=1,...,M$. 
%...(2) Building on (1): Grouping and considering competency standards w.r.t. 1st order `effects/outcomes' $O,S^F$ vs. 2nd order `causes/behaviors' $\Gamma_a, \Delta_a$. Could look at independently, but essential to look at both sets together (esp in nondeterministic setting) -- e.g. can behave optimally but still perform poorly (or vice versa) -- made right decisions with info available at time, or got lucky with wrong reasoning, etc. Competency self-assessment requires complete self-reflection in full context of understanding WHY behaviors are performed to define appropriate scope of meta-reasoning [Daw Neuro Psych]. So 1st/2nd order sets respectively look at answering what/where of competency indicator (i.e. what/where in task)  vs. how/why (did agent produce effects/outcomes it did), and changes to standards $\Sigma_i$ in this part essentially inform about expected capability. The conditional part of $f_i$ tells us who/when and changes to standards $\Sigma_i$ in this part informs about intrinsic capability (this is out of agent's control and part of definition of agent/task). 
%%...(3) Building on (2): block diagram provides semiformal functional structure to look at the `juices' available during auton dec making -- ingredients for the gravy, even in a non prob setting. structure points to low-hanging fruit to define competency indicator functions...

%%Remark on asymmetry: block diagram immediately allows us to see the asymmetry: expected capabilities depend on and are bounded by intrinsic capabilities. Expected capabilities in this sense are also easier to quantify/measure and potentially generalize in given context setting of fixed $C,A,E,\Theta,\Lambda_a$, whereas intrinsic ones are more abstract and trickier/more effort to define/generalize... comports with intuition/common sense: much easier to generalize expected car capabilities if we keep same type of car fixed for delivering passengers on same/similar highway environment and look at different outcome stats for safety, handling/control, traffic management, passenger comfort, fuel economy, etc. under variable lighting, weather, traffic, road conditions vs. trying to assess intrinsic algorithm capabilities by changing/vary car type and scenery and sensors and purpose from passenger delivery to cargo delivery and changing users/algorithm tuning knobs, etc. all at once. Thus referring back to broad vs. specific competencies: broad statements are usually speaking to intrinsic capabilities, but are by necessity informed by/extrapolated from/grounded in expected capabilities (despite the dependence of expected on intrinsic!). 

Finally, a probabilistic argument is now put forth to show how this computational view formally links together both expected and intrinsic capability assessments. 
From the Evaluator's standpoint, consider the probability distribution of obtaining a result $\sigma \in \mathbb{S}_i$ for $A$ under criterion $i$ relative to $\Sigma_i$. Since $f_i$ must be specified and evaluated relative to an evaluation context $(C,A,E,\Theta, \Lambda_a)$, the probability of the result $f_i(\cdots) = \sigma$ can be immediately related to a conditional distribution for expected capability (assuming for simplicity only one criterion $i$), 
\begin{align}
    p(\sigma|C,A,E,\Theta, \Lambda_a) = \frac{p(\sigma,C,\Theta, \Lambda_a|A,E)}{p(C,\Theta, \Lambda_a|A,E)},
    \label{eq:cond_sigma}
\end{align}
where $A$ and $E$ are fixed by the definition of the task and evaluation problem. 
From this, it follows $p(\sigma,C,\Theta, \Lambda_a|A,E) = p(C,\Theta, \Lambda_a|A,E) \cdot p(\sigma|C,\Theta, \Lambda_a,A,E)$, where the first term on the right-hand side denotes a prior distribution on the evaluation contexts for given $A$ and $E$. But for (\ref{eq:cond_sigma}) to be well-defined, it must also be the case that $p(C,\Theta, \Lambda_a|A,E)>0$; that is, $(C,\Theta,\Lambda_a)$ can only refer to evaluation contexts that are `not impossible'. Summing over these valid evaluation contexts yields
\begin{align}
    p(\sigma|A,E) = \sum_{C,\Theta, \Lambda_a} p(\sigma,C,\Theta, \Lambda_a|A,E) = \sum_{C,\Theta, \Lambda_a} p(C,\Theta, \Lambda_a|A,E) \cdot p(\sigma|C,\Theta, \Lambda_a,A,E),
    \label{eq:marg_sigma}
\end{align}
which is the distribution of $A$ achieving $f_i(\cdots)=\sigma$ in $E$, regardless of possible evaluation context. 
This gives a measure of intrinsic capability for $A$ in $E$ that depends on specifying the probabilities of realizing any possible evaluation context and expected capabilities for that context. Eq. (\ref{eq:marg_sigma}) also naturally comports with the idea discussed earlier that intrinsic capability assessments can be `atomically' built up from a suitably weighted average of expected capability assessments under all possible contexts. 
As such, eqs. (\ref{eq:cond_sigma}) and (\ref{eq:marg_sigma}) solidify the intuition that expected capability assessment is a computationally simpler and more tractable problem compared to intrinsic capability assessment. This follows not only since the latter subsumes the former, but also since it is non-trivial to come up with precise $p(C,\Theta,\Lambda_a|A,E)$ priors, even leaving aside the difficulty of comprehensively defining what information must go into $C$ and $E$ (whereas, formal methods tools exist which can precisely obtain $p(\sigma|C,\Theta,\Lambda_a,A,E)$ when $f_i, A,$ and $E$ have certain properties \nra{cite}). Thus, expected capability assessments are arguably the practical building blocks of computational competency evaluation.

\nra{could say something about a priori, in situ, post hoc assessments in terms of probabilistic prediction, filtering, smoothing distributions of eqs. (6) and (7)?? i.e. comes down to when is conditioning evidence becomes available in RHS of (6) relative to task execution -- Likewise for conditional term in (7)...}

\nra{honing in on this last major point: ingredients for report card and block are effects/causes $(O,S,\Gamma_a,\Delta_a)$ -- so now want to dive more deeply to examine what are the appropriate kinds of expected capability assessments and competency indicator functions for certain classes of rational goal-oriented agents doing decision-making under uncertainty?...} %%\nisar{need to make it a bit more explicitly clear earlier that eq. (1) is an expected assessment??}
%\nra{ideally would want to look at joint distribution of intrinsic and expected capabilities...can't really do this b/c of difficulty of looking over all contexts, possible types of agents, etc. -- so instead of looking at joint distribution, look at isolated conditional distributions of expected capabilities given intrinsic capability conditions -- in view of law of total probability, can then build up a complete picture under sufficiently broad coverage of intrinsic capability conditions to get approximate sense of `global' agent capabilities...} 

%\begin{itemize}
% \item Competency -- what is it? why do we care? define/discuss formal terms (A,C,R,O) comparative nature of our definition, i.e. relying on evaluation of outcomes attainable with current abilities as compared to an ideal set of outcomes under some given set of demands. Brett's def from slides: `The comparison of an outcome of interest O to a given `standard of competence' R, where O is produced by an agent A acting in a given context C.' Not saying what source of standard is, per se, but in our case it is defined by user/designer? Needs to be calculable from set of inputs that are available to an autonomous agent for it to do self-assessment and reporting. Connection to controllability (making `state' change to something more desirable -- change involves comparison of new to old state implicitly) and margins (degree to which achievement is possible, or effort/info is required) -- basis for argument for why comparison is fundamental to definition of competence?
% \item PUT IN BLOCK DIAGRAM FROM DRIVE
%%\item flavors of competency assessment: e.g. prospective/a priori, in situ, post hoc/retrospective -- what are the questions that need answers from some kind of computation?
%%\item relationship b/w competency and machine self-confidence ideas (in narrow/specific context of decision making under uncertainty) -- key point: taking the general concept of s/c given in prev section, must make it conceptually applicable to decision making problems, e.g. planning, etc. S/C oriented meta-reasoning aspect therefore means that agents don't just look at outcome of plans/actions/policies, etc. in relation to expected behavior or performance for particular instance of a task, but also need to look at what goes into those artifacts. 
%%\item the `arithmetic' of s/c: hierarchical argument in terms of conditional variables seems to be most natural way to go about this (also supported by Goodrich, et al's work as well as neurocogsci). More specifically: concept of `uncertainty in the process/uncertainty' is relevant 
%%\item Narrowing down to rational/goal-oriented agents operating under uncertainty, i.e. what kind of A,C,R,O are we interested in for this work -- competency of an MDP Agent: MDP gives prototype, but we can extend ideas beyond this, e.g. to MDP-adjacent (POMDP, RL, etc.) and non-Markov decision-making agents,etc. -- focus for this paper to make ideas concrete and clear: how do we apply ideas of competency to an MDP? Desiderata/thoughts experiments, contextual variances (e.g. driving up a mountain with a car vs. tank in snow), etc.
%%\item definition of MDPs and associated terminology (formally)
%%\item Meta-capabilities of an MDP (as distinct from capabilities expected from agent when it takes and strings together actions and evaluates its own state) -- factors of competency of an MDP associated with components of decision making process and FaMSeC block diagram...
%    \begin{itemize}
%        \item Effects of approximations
%        \item Validity of models
%        \item ramifications of uncertain outcomes
%        \item interpretation and mapping of user desires/demands to model, policy, outcome evaluation
%        \item influence of past experience or reference data
%    \end{itemize}
%\end{itemize}

==> competency_overview.tex <==
\subsection{Overview}\label{sec:overview}
Here we provide conceptual definitions helpful to introduce readers to the general ideas behind competency. These definitions are made more precise in Section~\ref{sec:formalization}

\begin{description}
\item[Competency:] The ability of an agent $A$ to achieve a desired set of outcomes and behaviors on a set of delegated tasks. Competency may be described in broad terms with regards to a generic set of capabilities (`The delivery drone can safely fly long distances and carry heavy packages in rough weather'), or contextualized to indicate specific  qualities, capabilities, or operational boundaries (`The drone can safely operate over a 5 mile range with a 2 kg payload when flying at 25 knots under 500 ft with winds under 10 knots'). In this work, we focus on competency statements of the latter variety.  %, although qualitative statements of the former kind could also be derived. %%, since these in principle appear to be sufficient for building statements of the former type. 
\item[Evaluator:] An entity external to the agent $A$ which is responsible for gauging $A$'s competency, using whatever information is available about $A$ and the delegated task at hand. 
The Evaluator could be a user, system designer, or computational entity, e.g. a separate metacognition module that monitors $A$, or even $A$ itself. 
In this view, the Evaluator relies upon on a set of \emph{competence standards} $\Sigma$, which specify desired outcomes and behaviors on the delegated task. 

\item[Competency Evaluation:] The generation of a competency statement regarding $A$ by an Evaluator's use of a competency indicator function $f$ to compare a set of outcomes of interest $O$ and behavioral signals $(S, \Gamma_a, \Delta_a)$ against a given set of competence standards $\Sigma$ (provided by the Evaluator), where $O$ and $(S, \Gamma_a, \Delta_a)$ are produced by $A$ acting in a given environment $E$ under a given task context $C$. Competency evaluation may occur before, during, or after a task is undertaken by $A$, and multiple competency statements can be generated via multiple functions $f_i$, for some collection of evaluation criteria $i=1,...,M$ with corresponding standards $\Sigma_i$. 
\end{description}

\nra{TODO: Give a more high-level/intuitive succinct breakdown of the general gist of the synthesis into generic framework -- breaking things down into 1st order (outcomes) and 2nd order effects(causes of behavior)...perhaps merge this with `Synthesis' part from before to shrink overall length and get to the punchlines faster?}

==> definitions.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\columnwidth]{figs/competency_definition.pdf}
\caption{Figure illustrating an agent acting within a given context to accomplish some outcome.}
\label{aen}
\end{figure}

To establish the idea of computational competency assessment in a more formal and principled way for algorithmic decision makers, some useful definitions are introduced. We begin with basic definitions for competency evaluation to ground other concepts and relationships. We then provide a synthesis of major elements of computational competency self-assessment and discuss the main insights from this setup, which forms the basis of our algorithmic competency self-assessment framework via machine self-confidence. Example applications are presented to highlight key concepts, and are revisited throughout the rest of the paper as various components of our self-assessment framework are considered in greater detail for autonomous decision-making under uncertainty. The case of a single autonomous agent is considered throughout for simplicity, but the concepts and ideas could also be reasonably extended to multi-agent settings. %%%\nra{ start putting running examples in this section (right after FaMSeC??), right after defs...could include a swarm as an agent perhaps?} 

%%\bi{Perhaps we could introduce two subsections here: 3.1) Overview, and 3.2) Elaboration (or Formalization, or something along those lines\ldots)}
\nra{TODO: (1) pare this section way down: pull out key point: can formally define what ingredients go into a computational competency evaluation (what is the signature required of such a function) and how these can manifest in real world -- all other details for technical abstract math stuff can go into an Appendix; (2) pare down variable def text with a TABLE; (3) provide simple pictorial examples to show what variables (from TABLE) and comp evals can mean for practical problems (e.g. helicopter example, robot doing some package delivery, swarm/multiple agents, etc.).}

\input{competency_overview.tex}
\input{competency_formalization.tex} % move more material into this file as appropriate

\subsection{Competency of Model-based Decision-Making Agents}
Justify why MDPs(POMDPs) are interesting, consider what's available within the framework that we just described. 

How to identify terms defined above (context, environment, agent, etc.) within a typical MDP?



==> figs/FaMSeC_math_commands.tex <==
%%%%% FaMSeC Math shortcut commands
% try to make this file somewhat `self-sustaining' so we can 
% use it in other places
\let\Bbbk\relax
\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{bm}

\DeclareMathOperator*{\argmax}{\arg\!\max}

\newcommand{\famsec}{FaMSeC}
\newcommand{\solve}{\ensuremath{\mathcal{S}}}
\newcommand{\solveopt}{\ensuremath{\mathcal{S}^*}}
\newcommand{\solvecand}{\ensuremath{\mathcal{S}^C}}
\newcommand{\solvetrust}{\ensuremath{\mathcal{S}^T}}
\newcommand{\taskclass}{\ensuremath{c_{\mathcal{T}}}}
\newcommand{\task}{\ensuremath{\mathcal{T}}}
\newcommand{\taski}{\ensuremath{\mathcal{T}_i}}
\newcommand{\taskN}{\ensuremath{\mathcal{T}_N}}
\newcommand{\rwd}{\ensuremath{\mathcal{R}}}
\newcommand{\rwdopt}{\ensuremath{\mathcal{R}^*}}
\newcommand{\rwdoptapprox}{\ensuremath{\widetilde{\mathcal{R}}^*}}
\newcommand{\rwdapprox}{\ensuremath{\widetilde{\mathcal{R}}}}
\newcommand{\rwdpredicted}{\ensuremath{\hat{\mathcal{R}}}}
\newcommand{\rwdcand}{\ensuremath{\mathcal{R}^C}}
\newcommand{\rwdcandsim}{\ensuremath{\widetilde{\mathcal{R}}^C}}
\newcommand{\rwdtrust}{\ensuremath{\mathcal{R}^T}}
\newcommand{\rwdtrusti}{\ensuremath{\mathcal{R}^T_i}}
\newcommand{\rwdtrustN}{\ensuremath{\mathcal{R}^T_N}}
\newcommand{\rwdtrustpredict}{\ensuremath{\hat{\mathcal{R}}^T}}
\newcommand{\rwdtrustipredict}{\ensuremath{\hat{\mathcal{R}}^T_i}}
\newcommand{\rwdtrustisim}{\ensuremath{\widetilde{\mathcal{R}}^T_i}}
\newcommand{\policy}{\ensuremath{\mathcal{\pi}}}
\newcommand{\policyopt}{\ensuremath{\mathcal{\pi^*}}}
\newcommand{\policytrust}{\ensuremath{\mathcal{\pi}^T}}
\newcommand{\policycand}{\ensuremath{\mathcal{\pi}^C}}
\newcommand{\surrogate}{\ensuremath{\mathcal{M}(\mathcal{T})}}
\newcommand{\surrogatearg}[1]{\ensuremath{\mathcal{M}(#1)}}
\newcommand{\xQ}{\ensuremath{x_Q}} %solver quality
\newcommand{\xO}{\ensuremath{x_O}} %outcome assessment
\newcommand{\xP}{\ensuremath{x_P}} %past performance
\newcommand{\xI}{\ensuremath{x_I}} %command interpretation
\newcommand{\xM}{\ensuremath{x_M}} %model validity
\newcommand{\xind}{\ensuremath{x_i}} % generic factor, would use \xi but it is taken
\newcommand{\xSC}{\ensuremath{x_{SC}} = \{\xI, \xM, \xQ, \xO, \xP \}}
\newcommand{\dkl}{\ensuremath{D_{KL}}}
\newcommand{\hell}{\ensuremath{H^2}}
\newcommand{\hellmet}{\ensuremath{\hell(P,Q)}}
\newcommand{\dmu}{\ensuremath{\Delta \mu}}
\def\-{\raisebox{.75pt}{-}} %short negative sign
\newcommand{\ri}{\ensuremath{R_{\infty}}}
\newcommand{\riref}{\ensuremath{\bar{R}_{\infty}}}
\newcommand{\pigeneric}{\ensuremath{\pi}}
\newcommand{\piapprox}{\ensuremath{\tilde{\pi}}}
\newcommand{\piopt}{\ensuremath{\pi^*}}
\newcommand{\picand}{\ensuremath{\pi^C}}
\newcommand{\pitrust}{\ensuremath{\pi^T}}
\newcommand{\pri}{\ensuremath{p(\ri)}}
\newcommand{\ppioptri}{\ensuremath{p_{\pi^*}(\ri)}}
\newcommand{\ppigenericri}{\ensuremath{p_{\tilde{\pi}}(R_{\infty})}}
\newcommand{\ppitrustpredict}{\ensuremath{\hat{p}_{\pi^T}(R_{\infty})}}
\newcommand{\ppicand}{\ensuremath{p_{\pi^C}(R_{\infty})}}
\newcommand{\ps}[1]{\ensuremath{p<#1}}
\newcommand{\pns}{\ensuremath{p>0.05}}
\newcommand{\cd}[1]{\ensuremath{d=#1}}
\newcommand{\Fratio}[4]{\ensuremath{(F_{#1,#2}=#3,\ps{#4})}}
\newcommand{\FratioCohen}[5]{\ensuremath{(F_{#1,#2}=#3,\ps{#4},\cd{#5})}}
\newcommand{\Frations}[3]{\ensuremath{(F_{#1,#2}=#3,\pns{})}}
\newcommand{\MSD}[2]{\ensuremath{(M=#1,SD=#2)}}
\newcommand{\CMSD}[3]{\ensuremath{(}Condition: #1;\ensuremath{M=#2,SD=#3)}}
\newcommand{\xQRR}{\ensuremath{\xQ(\rwdtrustpredict,\rwdcandsim)}}
\newcommand{\lwr}[1]{\ensuremath{L_{#1}}}
\newcommand{\upr}[1]{\ensuremath{U_{#1}}}
\newcommand{\flow}{\ensuremath{\lwr{\xind}}}
\newcommand{\fup}{\ensuremath{\upr{\xind}}}
\newcommand{\xMlow}{\ensuremath{\lwr{\xM}}}
\newcommand{\xMup}{\ensuremath{\upr{\xM}}}
\newcommand{\xIlow}{\ensuremath{\lwr{\xI}}}
\newcommand{\xIup}{\ensuremath{\upr{\xI}}}
\newcommand{\xPlow}{\ensuremath{\lwr{\xP}}}
\newcommand{\xPup}{\ensuremath{\upr{\xP}}}
\newcommand{\xQlow}{\ensuremath{\lwr{\xQ}}}
\newcommand{\xQup}{\ensuremath{\upr{\xQ}}}
\newcommand{\Upolicyopts}{\ensuremath{U^{*}(s)}}
\newcommand{\piopts}{\ensuremath{\piopt(s)}}
\newcommand{\emcts}{\ensuremath{e_{mcts}}}
\newcommand{\dmcts}{\ensuremath{d_{mcts}}}
\newcommand{\itsmcts}{\ensuremath{its_{mcts}}}
\newcommand{\rwdexit}{\ensuremath{rwd_{exit}}}
\newcommand{\rwdcaught}{\ensuremath{rwd_{caught}}}
\newcommand{\rwdsense}{\ensuremath{rwd_{sense}}}


==> measures.tex <==
\nra{NISAR TODO: split up into 3 new sections, one for OA, SQ, and then everything else - incorporate relevant running examples introduced from prev chapter into each}

Outline of key parts/points to drive into details:
\begin{itemize}
    \item go into details for indicators of  outcome assessment in depth - introduce via GOA (Jamison's thesis work), then narrow down to low-hanging fruit to reward-based formulation; include ideas from prospect theory here (Nick's recent work? illustrate in contrast to UPM/LPM?)
    \item go into details for indicators of solver quality -- again explain from general variable perspective, but illustrate via low-hanging fruit reward-based approach 
    \item give possible ideas for model quality (Luke Burks' surprise index approach for MDPs?), and motivation for interpretation and past history/data (how existing things like out of distribution measures could be useful, but would need to be tied to other factors potentially -- examples of how this might look conceptually as far as trends/boundary conditions from vignettes go?). 
\end{itemize}


Other things to discuss as well:
\begin{itemize}
    \item how to measure the accuracy of machine self-confidence reports according to proposed indicators or other ones? (e.g. Brier score for OA...)
    \item mention need for human subject tests and how this is already "out there" (Brett's thesis work and forthcoming other paper)
    \item `completeness' of factors? they may not cover everything, but they're pretty close/good. -- we are really only focusing on model-based decision making agents, and we are using a model of model-based agents to come up with estimates of competency (forecasting problem wrt 2nd order uncertainties). IE you can estimate competency/self-confidence if you define it like so (flow down from fundamental def  to mean gap between expectation and reality)...not necessarily a directly translation from estimation theory but an analog -- why is it/would it be different (why not just apply definition of estimator consistency directly)?
\end{itemize}


==> old_prelims.tex <==
The (5000 ft view of) problem of competency/proficiency self-assessment (brief relevant examples? ability to highlight shortcomings of different related approaches?)...need to sum up other background stuff from metacog/metareasoning, introspection, etc. and also more recent stuff on prof.SA + machine self-confidence (how to actually do it?? autonomously??), stat modeling/estimation, etc. and identify the gaps (synthesis of shortcomings and need for new framework/framing) --> where are we exactly, and why is it important for us to do what we're proposing? (bottom line: need machines to be able to identify their own limits when it comes to prob models for dec making under uncertainty...)
\begin{itemize}
    \begin{itemize}
        \item algorithmic assurances
        \item safe-rl
        \item explainable ai
        \item machine competency--proficiency self-assessment: related to but distinct from explainable ai
        \item machine self-confidence and relationship to competency/proficiency self-assessment (in broader terms, not specific to decision-making per se) -- cite prev work by Hutchins, etc. -- key idea:  machine self-confidence is a specific type of competency self-evaluation that reflects a particular kind of meta-knowledge and meta-analysis on part of machine as it pertains to a particular task, i.e. not general/global capability assessment that is agnostic of particular details of situation (e.g. deterministic reachability/controllability analysis) but an instance-based/ point-wise/case-driven evaluation that must be made in relation to expected behavior or performance while accounting for impacts of uncertainty/lack of knowledge (aleatoric or epistemic). Many ways this could be done for perception agents, etc. but no established way to do this for decision-making processes (focus of this work) -- but we're NOT trying to close the loop and improve behavior, just communicate with a (human) user/stakeholder
        \item meta-cognition/meta-reasoning
        \item introspective classifiers/ML
        \item relationship to psychological meaning/def of competency/proficiency (sports articles, Dunning-Kruger, models fo 2nd orer human uncertainty, etc)
        \item is it at all worth talking about concepts like advantage, critical states, etc. from RL/MDPs? in particular, how these differ from what we're looking for...most notably: can't just look at objective function for competency, esp if relevant things were not programmed in there in first place + many tasks too complex to be boiled down to a single number
    \end{itemize}
    \item MDPs: as a prototype for decision making autonomous agents, relationship to RL, POMDPs, etc. examples for dec-making under uncertainty (which we will examine more closely later/throughout)...pitfalls: how to self-assess/diagnose correctness?
    \item some sources of inspiration: KF example, expert systems literature (diagnostics/monitoring), concepts from control theory, etc. -- how different from what MDPs, etc. have to offer/work with...
\end{itemize}


==> relatedwork.tex <==
\nra{Tried to better organize and put more meat on bones here to get main argument + tone/flow going toward rest of later sections. Go back and polish/clean up prose here later.}
Overiew/roadmap: review of key concepts and related work on machine self-confidence and competency self-assessment. First begin with survey of important related ideas spanning a few major areas, mainly: human-machine/robot interaction; algorithmic metacognition/metareasoning, introspection, safety and explainability; and psychology. %Then go into preliminaries to focus on autonomous rational decision making agents that reason and act under uncertainty. 
 This all provides a basis for defining autonomous decision-making competency in rational agents that act under uncertainty in Sec. 3. 

\subsection{Trust and Algorithmic Assurances}
Quick framing of problem from trust and trust cycle relationship between human and AIA, per ACM 2019 paper. Discuss idea of how algorithmic assurances can be used to modulate/calibrate/adjust user expectations of robot partners -- spectrum of possible assurances from integral types (i.e. baked in behavior, such as legible motion planning) to non-integral/supplementary types (e.g. reporting of data). 

Assurance targets: competency as one aspect that can be informed in real time, along with predictability and reliability. Though cannot always cleanly separate these, competency assessment and reporting ideas has only received attention in recent years for sophisticated AI agents. Note that goal here is NOT to adapt the AIA, but rather to simply communicate assurances in form of assessment of capabilities relative to tasks at hand, to ensure that machine agents are used within their designed scope.  

\subsection{Machine Self-confidence and Proficiency Self-assessment}
Idea of `Machine self-trust'. Discuss definition and related work by Hutchins, Cummings, et al and others from AAAI 2015 workshop. Main takeaway: establishes machine s/c as a way of communicating capabilities to human stakeholders/users, but no unified mechanism for computing and very problem specific grounding of different ideas that are actually important to general autonomous systems.

Discuss recent/related work by Crandall, Goodrich, et al. and recent THRI paper. Main takeaway: gives taxonomy and some recent work talk about ways of computing monitors (Gautam ICRA 2022 -- assumption alignment idea closely related to GOA concept we discuss later on). But not specific to MDPs and does not explicitly consider/give computable metrics for higher level uncertainties in assessments (??), e.g. model and solver limits.  

\bi{perhaps cite paper from AAAI workshop}

\subsection{Algorithmic metareasoning, introspection, and explainability}
Ideas of enabling self-assessment and self-guided self-improvement in rational AI agents are not new -- Russell, many others since 1990's... more recently: Zilberstein et al for MDPs, and Griffiths et al for meta-RL. Key focus is on algorithmic adaptation.  Much less consideration and focus in these works given to idea of algorithmic assurances and trust cycle with human partners. Key idea here is bounded rationality: agent does not have infinite computing resources, so has limited capacity for self-knowledge/self-improvement, and therefore it can only think so hard to reach so many conclusions about itself in pursuit of rational goals. Also key are heuristics used to spot opportunities for self-improvement --- because of bounded rationality, agents can't know exactly how best to achieve better behavior, so they must rely on some kind of problem-specific heuristic evaluation mechanisms to determine how/when they can `do better'. Important takeaway is that there is no silver bullet answer -- furthermore, what metrics are algorithmically useful may only be appreciated by experts like system designers, i.e. they may not necessarily be useful or relatable/communicable to human user. \nra{add bit more here as/if needed?}

Introspection in robotics: Posner, others --- looking at ways robots can diagnose `complexity and difficulty' in different tasking situations, e.g. perception and classification. Does not necessarily extrapolate back to say anything about general robot competencies, and to date very little done on introspection of decision-making itself (mostly on perception side). \nra{Need to beef this up more with other updated references and takeaways...}

Control theory and safe RL: concepts of controllability/reachability and observability: in linear controls, defines capability of dynamical control system to achieve transfer between states in finite time and perfectly recover knowledge of unknown system states from finite set of observations. These are formed from mathematical models of dynamical systems and relate fundamentally to determining what a control system can/cannot theoretically achieve. Non-trivial to extend to non-linear and stochastic systems, but idea of `achievability' is central to machine s/c. Another important related concept from control theory is margin --- i.e. how robust is system to errors in modeling to avoid instability or severe degradation in performance? Greater margin implies greater confidence in deployment in real world. Computing such margins again non-trivial for AIAs, but idea is worth carrying forward in some more formal sense. 

For instance, this kind of thinking inspired safe RL and idea of shielding, etc. to establish an explicit boundary for control authority/capability.  Was derived from robust control literature idea of throttling control to maintain safety margins, so that agent has some guaranteed margin to recover if it does something unsafe/dumb while exploring. This is more of a forward-design idea to ensure safety: designer/agent explicitly limits itself to stay within some desired region that is already KNOWN to be safe/achievable -- can tell when it crosses a given line, but does not try to examine/reason about or assert/communicate knowledge of its ACTUAL limits/capabilities in particular circumstances. \nra{What more to say here?} Also again doesn't consider meta aspects or influences on capabilities, just looks at agent `as is'. \nra{add more on stuff from formal methods and reachability analysis?}

Explainability: Competency self-assessment is related to but distinct from XAI: specifically, the justification aspect of explainability is very important for making effective assurances that engender appropriate levels of human trust in AI agents (e.g. Bertram Malle's work). Many ideas have been proposed in XAI literature, e.g. critical states for MDPs -- framed in terms of problem and value function -- related to what we consider as outcome assessment, but doesn't necessarily scale well or work for online solvers, and says nothing about higher level layers of uncertainty, and does not provide competency statement in the end, esp cannot just look at obj function for competency if relevant aspects not programmed in there in first place AND if agent has incorrect policy/model for job. Also,  many tasks too complex to be boiled down to a single number --- competency assessment necessarily involves examining/considering some kind of trade space/Pareto front where a range of possible competency contexts can be established (i.e. can do task A if given resources X, but not if given resources Y). \nra{also mention two papers Brett flagged: (1) NeurIPS (?) paper on assessing whether reward/utility fxns are representative of task (related to point about boiling things down to single number -- MDP purists like Zach Sunberg may argue that MDP inappropriate otherwise); (2) Halpern 2018 work on blameworthiness -- reasoning about what agent actually can influence in probabilistic sense, link to causal reasoning...} 

\subsection{Neurocognitive Modeling and Psychology}
\nra{not quite sure where this belongs exactly...}
Major idea behind self-confidence in modeling self-assessment capability in human perceptual-motor tasks: self-confidence deeply tied to agent's introspection and understanding of second order uncertainty, i.e. uncertainty in uncertainty. Cite Daw, others: often people better at knowing how bad they are at low-level task than doing low-level task themselves. These ideas exist in realm of low level sensing/task execution as opposed to higher level reasoning and planning, but suggests an important resonance for ML/AI-based agents which nevertheless rely on common probabilistic frameworks for solving both high-level planning/reasoning problems and lower-level control/sensing problems, e.g. see proliferation of work on deep RL and perception work which looks at modeling epistemic as well as aleatoric uncertainty, as well as work on calibrating uncertainty (cite). Friston and others: Free energy minimization idea suggests that reducing model uncertainty/surprisal is important for `confident' behavior. 
Main takeaway: going beyond `raw' probability assessment values and looking at uncertainty in ingredients that inform those assessments gives pathway to enabling introspective proficiency self-assessments.   

Also relevant ideas about self-confidence in sports psychology, competency in business literature...Literature related to ``competency'' is mainly found in the business and management fields where ``core competencies'' \cite{Chouhan2014-ux} \bi{add some other citations of literature including education, and other, then transition to machine competency}.

Dunning-Krueger effect: perils of incorrectly calibrated confidence...

\subsection{Synthesis} \label{sec:synthesis}
%In summary: all these ideas touch on different aspects that are important to algorithmic machine s/c and competency self-assessment in decision making under uncertainty, but do not on their own provide a holistic approach to attacking the problem. Machine self-confidence is a specific type of competency self-evaluation that reflects a particular kind of meta-knowledge and meta-analysis on part of machine as it pertains to a particular task, i.e. not general/global capability assessment that is agnostic of particular details of situation (e.g. deterministic reachability/controllability analysis) but an instance-based/ point-wise/case-driven evaluation that must be made in relation to expected behavior or performance while accounting for impacts of uncertainty/lack of knowledge (aleatoric or epistemic).
\nra{TODO: Pare this section waaay down, possibly merge with Sec. 3.1/3.2, or just excise altogether}


Synthesizing insights from the aforementioned works reveals a few major points related to the question of how the competency of intelligent autonomous agents can be assessed computationally. 

Firstly, while there are many important aspects and concepts relevant to the  assessment of autonomous machine competency in specific settings, there is a need to combine these into coherent and practical computational frameworks that can span a broad range of applications. \nra{...SUCCESS MURI and metacog/metareasoning works represent step in these directions, but apparently overlook some aspects of things like dec making under uncertainty...}
    
Secondly, on the question of the computability of competency assessments, any such framework must be able to distinguish between different framings of and influences on agent capability. In particular, there is a difference between `intrinsic' capabilities determined by the set of possible problem settings and overall agent design, and `expected' capabilities determined by how specifically an autonomous agent is deployed and what specific behavior is demanded within a given problem setting. For instance, it is generally difficult for aircraft to fly safely in strong winds, bad weather, or compromised control conditions (damaged wing or control surfaces), regardless of the type of aircraft, pilot skill, instruments available, etc. In this domain, the intrinsic capability of a (non-)human pilot -- i.e. the absolute degree or range of possible agency for any agent -- is tied to factors beyond the agent's influence like weather conditions, vehicle design, the laws of physics, etc., rather than just the detailed agent design. Expected capabilities -- i.e. the demanded extent of agency relative to the situation at hand -- would include the agent's ability to maintain vehicle stability and control within its flight envelope subject to some expected range of disturbances, as well the ability to correctly perceive and process information in a timely manner to determine whether, when, and where it is safe and appropriate to execute maneuvers in given circumstances. 
As such, expected capabilities are tied to contextual assumptions related to intrinsic capabilities, while intrinsic capabilities must be consistent with expected capabilities across a range of contexts. 
Thus, to holistically answer questions about expected agent capabilities in situations that may or may not be in line with original design intentions, consideration must also be given to whether underlying assumptions about factors influencing intrinsic capabilities still hold, while some account must also be given for how expected capabilities `add up' to inform intrinsic ones.  Coming up with a way to account for, link, and assess factors related to intrinsic and expected capabilities poses a particularly interesting challenge from a computational perspective, which
will be discussed in the next section. 
%\nra{therefore, need to capture both -- only possible way to do so in real world problems is to look at expected capabilities in a given context, since impossible to look at all agents or all circumstances except for very simple toy/academic settings where this is inherently restricted...said differently, we wouldn't necessarily blame a pilot or call them incompetent if they crashed in bad weather -- depends on circumstances. On other hand, we are more inclined to question competency if they crashed in good weather, etc. i.e. if there was no reason for them to fail... the real point here: we need to understand intrinsic capabilities in case we get a question about expected capabilities which exceeds the original design -- i.e. can robot do something it wasn't originally designed for, but is intrinsically feasible? expected capability space could now expand...}

%%\nra{...towards 1st order task effects vs 2nd order behavioral causes...} 
Finally, it is clear that competency assessment requires evaluation of agent performance against a set of standards that are appropriate for a given context. From a computational point of view, autonomous agent performance can be divided into two categories of evaluable artifacts with corresponding sets of standards: \emph{task results} (assessing what the agent achieves), and \emph{resulting behaviors} (assessing how the agent achieves results). While each category could be examined independently, it is useful to examine both together to provide complete context for competency assessment. For non-deterministic settings in particular, optimal decisions can be made with resources and information available to the agent at the time, and yet still lead to poor task results. In such situations and in view of the need to provide algorithmic assurances to modulate trust, a useful computational approach to competency assessment should enable distinction between agents that are: intrinsically capable of performing tasks but which still consistently and predictably fail to meet expected capabilities in particular settings; intrinsically incapable and thus destined to fail no matter what; or fully capable but which get unlucky through chance occurrences. Conversely, if agents can succeed at non-deterministic tasks, competency assessment should be able to indicate whether (and under what conditions) agents are reliably/predictably competent vs. simply lucky. 
%\nra{Conversely -- if task is successful, want to be able to tell if agent was just lucky or if it can reliably/predictably be competent and under what conditions...}

